3D Gaussian Representations with Motion Trajectory Field for Dynamic Scene Reconstruction

This paper addresses the challenge of novel-view synthesis and motion reconstruction of dynamic scenes from monocular video, which is critical for many robotic applications. Although Neural Radiance Fields (NeRF) and 3D Gaussian Splatting (3DGS) have demonstrated remarkable success in rendering static scenes, extending them to reconstruct dynamic scenes remains challenging. In this work, we introduce a novel approach that combines 3DGS with a motion trajectory field, enabling precise handling of complex object motions and achieving physically plausible motion trajectories. By decoupling dynamic objects from static background, our method compactly optimizes the motion trajectory field. The approach incorporates time-invariant motion coefficients and shared motion trajectory bases to capture intricate motion patterns while minimizing optimization complexity. Extensive experiments demonstrate that our approach achieves state-of-the-art results in both novel-view synthesis and motion trajectory recovery from monocular video, advancing the capabilities of dynamic scene reconstruction.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> preamble.tex <==
\usepackage{subcaption}
\usepackage{subfig}
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sections/3_preliminary.tex <==
\section{Preliminary}\label{sec:preliminary}

\subsection{3D Gaussian Splatting}\label{sec:prel_gs}
3D Gaussian Splatting \cite{kerbl20233d} represents a static 3D scene using anisotropic 3D Gaussians optimized through differentiable rasterization for real-time, high-fidelity rendering. Each 3D Gaussian \(i\) has a center \(\mu_i\), a covariance matrix \(\Sigma_i\), an opacity \(\sigma_i\), and spherical harmonics (SH) coefficients \(h_i\). The opacity \(\alpha_i\) at any point \(\mathbf{x}\) is:
\begin{equation}
\alpha_i = \sigma_i \exp \left( -\frac{1}{2} (\mathbf{x} - \mu_i)^T \Sigma_i^{-1} (\mathbf{x} - \mu_i) \right).
\end{equation}

To facilitate the learning of 3D Gaussians, the positive semi-definite matrix \(\Sigma\) is divided into two learnable components: a scaling matrix \(S_i\) and a rotation matrix \(R_i\), in which \(S_i\) is a diagonal matrix and \(R_i\) is parameterized by a quaternion.

\begin{equation}
\Sigma_i = R_i S_i S_i^T R_i^T,    
\end{equation}


% rotation factor $\mathbf{r} \in \mathbb{R}^4$, and scaling factor $\mathbf{s} \in \mathbb{R}^3$

For rendering, 3D Gaussians are projected onto the 2D image plane. The 2D Gaussian center \(\mu_i^{2D}\) and covariance \(\Sigma_i^{2D}\) are computed using the viewing transformation \(W\), projection matrix \(K\), and Jacobian \(J\):

\begin{equation}
\mu_i^{2D} = \left(K \frac{W \mu_i}{(W \mu_i)_z}\right)_{1:2}; \Sigma_i^{2D} = \left(J W \Sigma_i W^T J^T\right)_{1:2, 1:2}.
\label{equ:gs_splatting}    
\end{equation}


After sorting the Gaussians in the depth order, the colour of pixel $p$ in the image plane, denoted as $C(p)$, is obtained through volume rendering:

\begin{equation}
C(p) = \sum_{i \in N} c_i \alpha_i^{2D} \prod_{j=1}^{i-1} (1 - \alpha_j^{2D})
\label{equ:gs_rendering}
\end{equation}


\noindent where \(c_i\) is the RGB color from SH coefficients and \(\alpha_i^{2D}\) is the 2D opacity.In summary, 3D Gaussian Splatting combines efficient rasterization and differentiable rendering to achieve high-fidelity, real-time novel view synthesis, making it a powerful technique for static scene representation.



\subsection{3D points in Trajectory Space}\label{prel_trajectory_space}

All deformable 3D points can be represented into low-rank trajectory space~\cite{akhter2008nonrigid}. To represent the structure at a specific time $t$, we organize the 3D coordinates of the points into a matrix $\boldsymbol{x}^t \in \mathbb{R}^{3 \times P}$,
% \[
% S(t) = \begin{bmatrix} \mathbf{x}_{t1} & \mathbf{X}_{t2} & \cdots & \mathbf{X}_{tP} \end{bmatrix},    
% \]
\begin{equation}
\boldsymbol{x}^t = \begin{bmatrix} x_{t1} & x_{t2} & \cdots & x_{tP} \end{bmatrix},    
\end{equation}

\noindent where ${x}_{ti} \in \mathbb{R}^3$ denotes the 3D coordinates of point $i$ at time $t$. The complete time-varying structure is represented by concatenating these instantaneous structures into $X \in \mathbb{R}^{(N \times 3) \times k}$:

% \begin{equation}
% S = \begin{bmatrix} S(1) \\ S(2) \\ \vdots \\ S(F) \end{bmatrix} = \begin{bmatrix} \mathbf{X}_{11} & \mathbf{X}_{12} & \cdots & \mathbf{X}_{1P} \\ \mathbf{X}_{21} & \mathbf{X}_{22} & \cdots & \mathbf{X}_{2P} \\ \vdots & \vdots & \cdots & \vdots \\ \mathbf{X}_{F1} & \mathbf{X}_{F2} & \cdots & \mathbf{X}_{FP} \end{bmatrix}.    
% \end{equation}


\begin{equation}
X = \begin{bmatrix} \boldsymbol{x}^1 \\ \boldsymbol{x}^2 \\ \vdots \\ \boldsymbol{x}^N \end{bmatrix} = \begin{bmatrix} x_{11} & x_{12} & \cdots & x_{1P} \\ x_{21} & x_{22} & \cdots & x_{2P} \\ \vdots & \vdots & \cdots & \vdots \\ x_{N1} & x_{N2} & \cdots & x_{NP} \end{bmatrix}.    
\end{equation}

The row space of this matrix represents the shape space~\cite{xiao2004closed}, while the column space is referred to as the trajectory space. For the shape and motion recovery, the structures are usually effectively represented using $k$ ($k$ < $P$) basis shapes~\cite{torresani2008nonrigid}, since the trajectory space holds a dual relationship with the shape space, the trajectory space can be equivalently represented with other $k$ basis trajectory vectors. To express the time-varying structure using trajectory bases, we view the structure as a set of trajectories ${T}_i \in \mathbb{R}^{N\times3}$:

\begin{equation}
T_i = \begin{bmatrix} x_{1i} & x_{2i} & \cdots & x_{Fi} \end{bmatrix}^T.
% \mathbf{T}_i = [\mathbf{X}_{1i},\space \mathbf{X}_{2i},\space \hdots,\space \mathbf{X}_{Fi} ]^T.
\end{equation}

Each trajectory ${T}_i$ can be described as a linear combination of basis trajectories:

\begin{equation}
T_i = \sum_{j=1}^k a_{ij} {\Theta}_j,
\end{equation}

\noindent where ${\Theta}_j \in \mathbb{R}^{N\times 3}$ is a basis trajectory, and $a_{ij}$ are the coefficients corresponding to that basis vector. The time-varying structure matrix $X$ can then be factorized into an inverse projection matrix ${\Theta} \in \mathbb{R}^{(N \times 3) \times k}$ and a coefficient matrix $A \in \mathbb{R}^{k \times P}$:

\[
X = {\Theta} A,
\]

where $A = \begin{bmatrix} A_1 & A_2 & \cdots & A_P \end{bmatrix}$, \[
A_i = \begin{bmatrix} a_{i1} & a_{i2} & \cdots & a_{ik} \end{bmatrix}^T, \quad {\Theta} = \begin{bmatrix} {\Theta}_1 & {\Theta}_2 & \cdots & {\Theta}_k \end{bmatrix}.
\]


The principal benefit of the trajectory space representation is that a basis can be pre-defined and can compactly approximate most real trajectories. Various bases such as the Hadamard Transform, Discrete Fourier Transform, and Discrete Wavelet Transform~\cite{wang2021neural, li2024generative} can all represent trajectories in an object-independent manner. This prior information will relieve the burden of optimizing the motion of 3D points in a dynamic scene. In this paper, we use the Discrete Cosine Transform (DCT) basis to initialize all basis trajectories, allowing optimization with a good initialization.

==> sections/4_method.tex <==
\section{3DGS in trajectory space}
Given a sequence of images from a dynamic scene with frames ($I_1$, $I_2$,...,$I_N$), and known camera parameters, our method aims to synthesize the novel-view image at any time point to recover the geometric dynamic, such as point trajectory.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/framework.pdf}
    \caption{The pipeline of our framework. 3DGS at time $t$ are transformed from global 3DGS using learnable motion bases ($\theta, \lambda, \eta$) and trajectory coefficients ($\sigma, \beta, \gamma$). Projection, density control, and Gaussian rasterization follow original paper~\cite{kerbl20233d}.}
    \label{fig:enter-label}
\end{figure*}

\subsection{3D Gaussians in trajectory space}
3D Guassians~\cite{kerbl20233d} was originally designed to represent static scenes. To extend its capabilities for dynamic scenes, we model the dynamics using a motion trajectory field. We assume a set of compact and moving 3D Gaussian points represents the dynamic scene, where each point follows a trajectory across all time frames. Each 3D Gaussian point has a time-varying covariance matrix but a time-invariant color coefficient (i.e., spherical harmonics). For the time-varying structure, we define a global reference point $x^{\star}_i \in \mathbb{R}^3$ for each trajectory $T_i$, which represents the global position of the point throughout the entire sequence. The global reference point $x^{\star}_i$ can be the initial position or a point in the middle of the trajectory $T_i$, differing from points in canonical space~\cite{pumarola2021d,yang2024deformable,liu2024modgs}. There are several reasons for defining the global reference point $x^{\star}_i$: 1) It helps mitigate global offsets by representing structures relative to global points, leading to more accurate and stable reconstructions; 2) Global points can be flexibly selected or learned for different types of motion and deformation; 3) Global points are useful for adaptive density control in 3DGS during optimization, helping prune transparent Gaussian points while densifying points in high-frequency areas. By decoupling global points and focusing on relative structures, we achieve a more robust and accurate process for deformation reconstruction.
% are designed for representing static scenes. We model the dynamics with a motion trajectory field to extend its capabilities for dynamic scenes. We assume that there is a set of compact moving 3D Gaussian points for representing the dynamic scene, and each 3D Gaussian point has a trajectory across all time-frames with time-varying covariance matrix but time-invariant colour coefficient (i.e. spherical harmonics). For the time-varying structure, we define a global reference point $g_i \in \mathbb{R}^3$ for each trajectory $T_i$ which represents the global position of this point across the entire sequence, and global reference point $g_i$ can be the initial point or point in the middle of entire trajectory $T_i$. There are several motivations behind defining global reference point $g_i$: 1), it helps to mitigate global offset by representing the structure relative to global points, leading to more accurate and stable reconstructions; 2). global points can be appropriately selected or learned to various types of motions and deformations, and the reconstructed points remain consistent with the global structure of the object throughout the sequence; 3). global points can be used in the adaptive density control in 3DGS during optimization, which can prune transparent Gassain points and also densify the Gaussian in high-frequency areas.  Therefore, by decoupling the global points and focusing on the relative structures, we can achieve a more robust and accurate process of deformation reconstruction. \color[red]{Explain the global points are different from canonical space, Gloabl points are explicitly correspond to any timestep but is just a virtual space that contains the canonical locations of all Gaussians.

We model the dynamic scene using relative time-varying structures. The relative position of the $i$th 3D Gaussian at time $t$ is given by $\Delta x_i^t = x_i^t - {x}^{\star}_i $, where $x_i^t$ is the center of the $i$th 3D Gaussian. Therefore, the relative trajectory of the $i$th 3D Gaussian is $\Delta T_i = [\Delta x_i^0, \Delta x_i^1, \dots, \Delta x_i^N]^{\tran}$, and the relative motion trajectories for all 3D Gaussian points can be represented as $\Delta T = [\Delta T_0, \Delta T_1, \dots, \Delta T_P] \in \mathbb{R}^{3N\times P}$. The relative trajectory of the $i$th point can be expressed as a linear combination of basis trajectories: $\Delta T_i = \sum_{j=1}^{k} {\sigma}^x_j({x}^{\star}_i)  \theta_j$, where $\theta_j \in \mathbb{R}^{N}$ are the trajectory basis vectors over all time frames, $\theta_j = [\theta_j^0, \theta_j^1, \dots, \theta_j^N]^{\tran}$, and ${\sigma}^x_j({x}^{\star}_i) \in \mathbb{R}^3$ are the trajectory coefficients modeled with MLPs and shared across all time frames. All global points are detached when inputted into the motion trajectory field, without background propagation. For the $i$th 3D Gaussian point at time $t$, its relative and global positions can be represented as:

\begin{equation}
\centering
\Delta x_i^t  = \sum_{j=1}^{k} {\sigma}_j({x}^{\star}_i) \theta_j^t 
\label{equ:1}
\end{equation}

\begin{equation}
 x_i^t  = {x}^{\star}_i + \sum_{j=1}^{k} {\sigma}_j({x}^{\star}_i) \theta_j^t   
 \label{equ:2}
\end{equation}


We represent scene motion using a motion trajectory field, described through learnable basis functions. For each 3D Gaussian point, we encode its trajectory coefficients with an MLP $\mathcal{F}_{tc}$, as follows:

\begin{equation}
\{\sigma_j(x^{\star}_i)\}_{j=1}^k = \mathcal{F}_{tc}(\mathcal{G}({x}^{\star}_i))
\end{equation}


where $\sigma_j^k \in \mathbb{R}^3$ are basis coefficients (separate for $x$, $y$, and $z$) and $\mathcal{G}$ represents positional encoding. We choose $k=40$ basis functions. The encoding function $\mathcal{G}$, with linearly increasing frequency, is expressed as:

\begin{equation}
\mathcal{G}({x}^{\star}_i) = \left( \sin(2^k \pi {x}^{\star}_i), \cos(2^k \pi {x}^{\star}_i) \right)_{k=0}^{L-1}
\end{equation}


where $L=12$ for encoding global reference point ${x}^{\star}_i$. This choice is based on the assumption that scene motion tends to occur at low frequencies~\cite{zhang2021consistent}. 


The global learnable motion basis, $\{\theta_j^t\}_{j=1}^k$, where $\theta_j^t \in \mathbb{R}$, is introduced to replace the trajectories basis in the original trajectory space~\cite{akhter2008nonrigid}. These bases span every time step $t$ of the input video and are optimized jointly with the MLP. Similarly with~\cite{wang2021neural, li2023dynibar}, we initialize the basis $\{\theta_j\}_{j=1}^k$ using the DCT basis, but fine-tune it during optimization along with other components. This fine-tuning is necessary because a fixed DCT basis often fails to capture the wide range of real-world motions~\cite{li2023dynibar}. The global reference points ${x}^{\star}_i$ are initialized using points from COLMAP~\cite{schoenberger2016sfm}, a standard procedure in 3DGS~\cite{kerbl20233d}.


Using ~\cref{equ:1} and~\cref{equ:2}, we can generate all Gaussian central points across all time frames, ${X} = [\boldsymbol{x}^1, \boldsymbol{x}^2, ...,\boldsymbol{x}^N]{T} \in \mathbb{R}^{(N\times 3)\times P}$, each row corresponds to all points at a single time frame, while each column represents the trajectory of a point. This motion trajectory field models the dynamic 3D Gaussian points. However, we observed that if each trajectory shares the same covariance across all time frames, using only a time-varying Gaussian centre is insufficient to effectively model dynamic scenes. Since 3DGS inlciudes anisotropic covariance, each Gaussian may exhibit temporally different rotations to capture dynamic geometry and appearance changes. To better model scene deformations, we extend the motion trajectory field (~\cref{equ:1} and~\cref{equ:2}), to also account for time-varying covariance $\Sigma_i = \boldsymbol{r}_i \boldsymbol{s}_i \boldsymbol{s}_i{\tran} \boldsymbol{r}_i{\tran}$~\cite{kerbl20233d} as the following equations:

\begin{equation}
\centering
s^t_i  = {s}^{\star}_i + \sum_{j=1}^{l} {\beta}_j({x}^{\star}_i) \lambda_j^t 
\end{equation}

\begin{equation}
r^t_i  = {r}^{\star}_i + \sum_{j=1}^{m} {\gamma}_j({x}^{\star}_i) \eta_j^t
\label{equ:scale}
\end{equation}

To simplify the model,  we keep opacity and radiance time-invariant, sharing them across all times and global reference points. The geometrical structure and covariance are time-varying, but each trajectory shares the same spherical harmonics coefficients, as the covariance and central points already account for changes in viewing perspectives over time. For the Gaussian $i$ at time $t$, we can obtain its Gaussian primitives \(\{x^t_i, s^t_i, r^t_i, \alpha_i, c_i\}\). By applying rendering equations from~\cite{kerbl20233d}, we can render the image at any time frame.


\subsection{Static and dynamic separation}

We assign an additional indicator parameter to each 3D Gaussian primitive to represent its states (static or dynamic). This distinction allows us to select dynamic Gaussian points for supervising the motion field. When modeling entire dynamic scenes using an implicit deformation field~\cite{yang2024deformable}, we observed that the static part can mistakenly acquire trajectories (see~\cref{fig:mask_img}). This not only harms novel-view synthesis for the static part but also introduces noisy supervision during training neural motion field. To address this, we assign a continuous parameter \(p \in [0, 1]\) to indicate the probability of a Gaussian primitive belonging to either the static background or dynamic foreground. Ideally, dynamic Gaussians in the foreground should have \(p = 1\), while others in the background should have \(p = 0\). Thus, the parameters of each 3D Gaussian primitive are extended to \(\{x^t_i, s^t_i, r^t_i, \alpha_i, c_i, p_i\}\). We render a static/dynamic segmentation mask ($\mathcal{\hat{M}}$) using volume rendering by replacing the $c_i$ with $p_i$ in rendering equations~\cite{kerbl20233d}. A pseudo-segmentation mask ($\mathcal{M}$) for dynamic objects is generated using segment and tracking anything~\cite{kirillov2023segment, ke2024segment, yang2023track}. The segmentation loss can be obtained as follows:



\begin{equation}
    \mathcal{L}_{m} = ||\mathcal{\hat{M}}  - \mathcal{M}||^2
\end{equation}

When rendering the segmentation map, Gaussian attributes of location, covariance, and opacity are detached without gradient, so that this loss only optimizes its state probability \(p_i\). We set a high threshold (0.8) for selecting the static Gaussian to mitigate the impact of segmentation errors on rendering and motion modelling, as it is observed that the motion field can model static background but not the other way around. The parameter \(p_i\) indicates whether a Gaussian is dynamic. When the model is well-optimized, \(p_i\) should be either \(0\) or \(1\), based on which we design the point-wise loss \(\mathcal{L}_{3mr}\) to force each Gaussian to have only one state. We add this loss at the late stage of the training process.


\begin{equation}
    \mathcal{L}_{3mr} = {\textstyle\footnotesize \frac{1}{k} \sum_{i=1}^{k}} -\left(p_i \log (p_i) + (1 - p_i) \log (1 - p_i)\right)
\end{equation}



\subsection{Motion regularization}
In the motion trajectory field, each point only provides location-dependent coefficients and all points share the same global motion basis which provides a weak prior on a smooth trajectory. To inject physical-based priors into the motion trajectory field, we apply the as rigid as possible loss~\cite{kumar2017monocular, luiten2023dynamic}, $\mathcal{L}^{\text{arap}}$, to achieve the temporal smoothness. We assume that each Gaussian and their neighboring Gaussian points should follow rigid transformation of the coordinate system cross two timesteps. The $\mathcal{L}^{\text{arap}}$ is defined as:
\begin{equation}
\begin{aligned}
\mathcal{L}_{arap} = \frac{1}{k|\mathcal{S}|} \sum_{i \in \mathcal{S}} \sum_{j \in \text{knn}_{i}}  &  w_{i,j} \| ( x_{j}^{t-1} - x_{i}^{t-1}) - \\ & r_{i}^{t-1} (r_{i}^t)^{-1}( x_{j}^t - x_{i}^t) \|_2       
\end{aligned}
\end{equation}

We randomly select $\mathcal{S}$ points to enforce the $\mathcal{L}^{\text{arap}}$, and for each selected point, a set of neigbhoring Gaussians are selected for it using the k-nearest neighboring (knn), and the loss is down-weighted by an isotropic Gaussian weighting factor:
\[
w_{i,j} = \exp\left( -\rho_w \| x_{j}(t) - x_{i}(t) \|_2^2 \right)
\]

We proposed a spatial smoothness loss to enforce smoothness over neighbouring spatial locations. We apply a perturbing $\epsilon$ on the input global points $x^{\star}$ and encourage the location-dependent attributes at location ${x}^{\star}_i + \epsilon$ to be consistent with ${x}^{\star}_i$. The spatial smoothness term is:

\begin{equation}
\begin{aligned}
    \mathcal{L}_{sp} = & \| {\sigma}_j({x}^{\star}_i) - {\sigma}_j({x}^{\star}_i + \epsilon) \|_2  + \\  
                     & w_{\beta} \| {\beta}_j({x}^{\star}_i) - {\beta}_j({x}^{\star}_i + \epsilon) \|_2  +  \\
                   & w_{\gamma} \| {\gamma}_j({x}^{\star}_i) - {\gamma}_j({x}^{\star}_i + \epsilon) \|_2    
\end{aligned}
\end{equation}


\noindent where the perturbing value's magnitude is adaptively set according to the scale of the scene, i.e., $\epsilon = 0.001*scale$, and $w_{\beta}$ and $w_{\gamma}$ are corresponding weighting factor for rotation and scale.

% Notably, the perturbing value's magnitude is adaptively set according to the number of total frames, i.e., $\epsilon = 0.1 / \text{frames}$.

% The deformation between two consecutive timestamps is locally and globally as rigid as possible, so the deformation is not arbitrary but regular and rigid. 

All these motion regularisers are applied only on dynamic Gaussian points using the foreground/background mask. We observe that dynamic Gaussian point tends to have a larger gradient flow than static points, since dynamic region has a large photometric loss and is also constrained with motion regularisers. If we apply the similar density control mechanism to both points, this can cause over-dense dynamic point, therefore, we set a large gradient threshold for densifying the dynamic points.

% \subsubsection{Adaptive Control Points} dynamic and static points are bounded to different control mechanisms.s

% \subsection{Optimization}

When the model is well optimized, we can render the image with the learned Gaussian primitives \(\{\mathbf{x}^*_i, \mathbf{s}^*_i, \mathbf{r}^*_i, \alpha_i, c_i, p_i\}\) with trajectory motion field only applied on dynamic Gaussian points. With the rendered images, we can caluclate the Photometric loss $\mathcal{L}_{pho}$, which is the same as~\cite{kerbl20233d}. Therefore, our final loss to optimize the model is as follow: 
\begin{equation}
\mathcal{L} =  \mathcal{L}_{pho} + \mathcal{L}_{m} + \mathcal{L}_{3mr} +  \lambda_a\mathcal{L}_{arap}  + \lambda_s\mathcal{L}_{sp}   
\end{equation}



